Search for top quark decays $t\rightarrow qH$ with $H\to\gamma\gamma$ using the ATLAS detector

A search is performed for flavour-changing neutral currents in the decay of a top quark to an up-type ($c, u$) quark and a Higgs boson, where the Higgs boson decays to two photons. The proton-proton collision data set used corresponds to 4.7 fb$^{-1}$ at $\sqrt{s}$ = 7 \tev\ and 20.3 fb$^{-1}$ at $\sqrt{s}$ = 8 \tev\ collected by the ATLAS experiment at the LHC. Top quark pair events are searched for in which one top quark decays to $qH$ and the other decays to $bW$. Both the hadronic and the leptonic decay modes of the $W$ boson are used. No significant signal is observed and an upper limit is set on the $t\rightarrow qH$ branching ratio of 0.79% at the 95% confidence level. The corresponding limit on the $tqH$ coupling combination $\sqrt{\lambda_{tcH}^{2} + \lambda_{tuH}^{2}}$ is 0.17.

==> acknow.tex <==
% CHECK THAT IT IS UPDATED

We thank CERN for the very successful operation of the LHC, as well as the
support staff from our institutions without whom ATLAS could not be
operated efficiently.

We acknowledge the support of ANPCyT, Argentina; YerPhI, Armenia; ARC,
Australia; BMWF, Austria; ANAS, Azerbaijan; SSTC, Belarus; CNPq and FAPESP,
Brazil; NSERC, NRC and CFI, Canada; CERN; CONICYT, Chile; CAS, MOST and
NSFC, China; COLCIENCIAS, Colombia; MSMT CR, MPO CR and VSC CR, Czech
Republic; DNRF, DNSRC and Lundbeck Foundation, Denmark; ARTEMIS, European
Union; IN2P3-CNRS, CEA-DSM/IRFU, France; GNAS, Georgia; BMBF, DFG, HGF, MPG
and AvH Foundation, Germany; GSRT, Greece; ISF, MINERVA, GIF, DIP and
Benoziyo Center, Israel; INFN, Italy; MEXT and JSPS, Japan; CNRST, Morocco;
FOM and NWO, Netherlands; RCN, Norway; MNiSW, Poland; GRICES and FCT,
Portugal; MERYS (MECTS), Romania; MES of Russia and ROSATOM, Russian
Federation; JINR; MSTD, Serbia; MSSR, Slovakia; ARRS and MVZT, Slovenia;
DST/NRF, South Africa; MICINN, Spain; SRC and Wallenberg Foundation,
Sweden; SER, SNSF and Cantons of Bern and Geneva, Switzerland; NSC, Taiwan;
TAEK, Turkey; STFC, the Royal Society and Leverhulme Trust, United Kingdom;
DOE and NSF, United States of America.

The crucial computing support from all WLCG partners is acknowledged
gratefully, in particular from CERN and the ATLAS Tier-1 facilities at
TRIUMF (Canada), NDGF (Denmark, Norway, Sweden), CC-IN2P3 (France),
KIT/GridKA (Germany), INFN-CNAF (Italy), NL-T1 (Netherlands), PIC (Spain),
ASGC (Taiwan), RAL (UK) and BNL (USA) and in the Tier-2 facilities
worldwide.

